SLO-Aware Task Offloading within Collaborative Vehicle Platoons

In the context of autonomous vehicles (AVs), offloading is essential for guaranteeing the execution of perception tasks, e.g., mobile mapping or object detection. While existing work focused extensively on minimizing inter-vehicle networking latency through offloading, other objectives become relevant in the case of vehicle platoons, e.g., energy efficiency or data quality for heavy-duty or public transport. Therefore, we aim to enforce these Service Level Objectives (SLOs) through intelligent task offloading within AV platoons. We present a collaborative framework for handling and offloading services in a purely Vehicle-to-Vehicle approach (V2V) based on Bayesian Networks (BNs). Each service aggregates local observations into a platoon-wide understanding of how to ensure SLOs for heterogeneous vehicle types. With the resulting models, services can proactively decide to offload if this promises to improve global SLO fulfillment. We evaluate the approach in a real-case setting, where vehicles in a platoon continuously (i.e., every 500 ms) interpret the SLOs of three actual perception services. Our probabilistic, predictive method shows promising results in handling large AV platoons; within seconds, it detects and resolves SLO violations through offloading.

==> sections/2_preliminaries.tex <==
% This section provides a more detailed description of the use case we address in this paper and the formal underlying problem, including the respective concepts and definitions used throughout the paper. Apart from that, this section also presents a number of tools and techniques that will be applied in Section~\ref{sec:methodology} to learn and estimate the SLO fulfillment of offloading operations.

\subsection{Bayesian Networks}
\label{subsec:background}


Bayesian Networks (BNs), as applied by Pearl~\cite{pearl_causal_2009}, are structural causal models encoded as Directed Acyclic Graph (DAG).
Nodes in a BN represent random variables (e.g., $cpu$); an edge between two variables (e.g., $cpu \rightarrow energy$) indicates conditional dependency, i.e., $cpu$ influences the states of $energy$. 

To model real-world processes and the probabilities of different system states, numerous works ~\cite{odiathevar_bayesian_2022,tasoulas_bayllocator_2012,togacar_detecting_2022}, trained BNs from historical observations (i.e., metrics).
Thus, given historical observations, BNs can answer how likely it is to observe a specific system state at runtime.
Spinning this thought further, the authors of \cite{sedlak_designing_2023,sedlak_controlling_2023} applied BNs to predict SLO fulfillment of microservices.
In particular, they constructed SLOs around BN variables, e.g., $\textit{energy} \leq 10 W$, which means that the SLO is fulfilled for any state of \textit{energy} that fulfills the equation. 

In the context of this work, we use BNs to interpret the SLO fulfillment during service execution, which requires training a dedicated BN for each service and vehicle type; we call this an SLO interpretation (SLO-I) model. Given the model $m$, agents predict the SLO fulfillment for a set of SLOs ($Q$) through $\texttt{INFER}(m, Q, C)$, where $Q$ and $C$ are SLOs and constraints defining the service execution.

As new observations ($O$) are received, the BN must be retrained to ensure that inferred probabilities remain accurate; we limit this process to the conditional probabilities of the BN and leave the structure untouched. Hence, $\texttt{PARL}(m,O)$ can be used to update the model with new observations.


==> sections/proposal.tex <==
\subsection*{Problem Description}

Autonomous vehicles are commonly equipped with edge devices that allow them to run powerful computations locally, e.g., video detection or point cloud processing. However, when choosing which device to embed in a vehicle, the default strategy is selecting one that performed well during experiments, but without understanding in-depth how much of these resources are essential to satisfy each task's requirements. The conservative choice is to rely on more powerful devices that are guaranteed to fulfill requirements, which increases the overall price of vehicles considerably, while its operation drains the device battery.
% \tmi{such vehicles must economize their battery usage by limiting their local computations to the minimum.} 
Without knowing how much resources a task would consume, offloading it to another device also jeopardizes its regular operations. This becomes graver when we consider that vehicles with mixed capabilities, e.g., due to different levels of autonomous driving, can have different processing hardware installed: given two vehicles for which we know only for the first how the task would perform, it is not possible to directly infer how it would perform on the second one, which impedes potential task offloading. Furthermore, existing research views offloading as a one-shot operation, though the target destination is not immediately guaranteed to fulfill processing requirements, showing the need for graceful offloading.

\ins{What is the underlying (combinatorial) problem? Why do we choose MKP and AIF as methods and not xyz other applications?}

Autonomous vehicles have limited capabilities for local processing; in case a vehicle wants to execute a service (i.e., computer vision or other perception tasks) that surpasses its capabilities or available resources, this likely infringes the QoS and QoE (e.g., processing latency or data quality) of this service, or existing services running there. While there exist options to offload computation to nearby RSUs or other vehicles in close vicinity, these mechanisms consider only networking aspects such as changes in networking latency caused by offloading. The problem that persists is that offloading mechanisms have little understanding of whether a target host disposes of sufficient resources to fulfill all its services' requirements. Furthermore, the underlying combinatorial problem, i.e., assigning $n$ services to $m$ hosts so that requirements are optimized, is NP-hard; hence, exhaustively comparing $m^n$ deployment combinations is impractical due to (1) the exponential solution space, (2) the computational overhead of empirically evaluating deployments, and (3) the fact that complex systems can change over time, making it a necessity to retrain or reevaluate the solutions.

\subsection*{Vision}

Vehicles form a cluster or platoon of nearby devices, which is led by an elected platoon leader. Perception tasks (or utility services) that vehicles want to execute (e.g., video processing) can be offloaded to other vehicles, even though executing the service to a satisfying degree would have exceeded its capabilities. The leader periodically evaluates whether the platoon performs well (i.e., in terms of SLOs) and reassigns tasks between the vehicles according to its understanding. When vehicles join or leave the platoon, services are reassigned among the remaining members; to find satisfactory assignments regardless of these changes, the leader actively explores the solution space. Thus, the leader maintains an overview of which vehicles (or rather their processing devices) are capable of running different tasks and how much energy this would consume.

\subsection*{Methodology}

Assuring the SLO fulfillment of offloaded tasks requires the platoon leader to understand (\textbf{I}) the degree to which different edge devices can fulfill SLOs; if the current level of knowledge is insufficient (e.g., nonexistent or outdated) the leader has to gain further insights by testing deployments on candidate devices. Further, the leader must know (\textbf{II}) the amount of resources that this task consumes at the potential location; through periodical reports from platoon members, it becomes evident how much resources currently executed services consume and how much resources would be available for offloaded tasks.

The underlying combinatorial of optically assigning services to vehicles is modeled as a Multiple Knapsack Problem (MKP) with the following characteristics: (1) each vehicle represents a knapsack that (2) has a capacity according to its hardware capabilities; it is possible to (3) model different capabilities (e.g., CPU or GPU) with different constraints, which are (4) allocated to a service according to its computational demand. Adding a service to a vehicle (5) provides value equivalent to the expected SLO fulfillment, which (6) can be different according to which vehicle the service is assigned to. The MKP is (7) bounded so that each service can be assigned at most one time to one knapsack. Noteworthy, there should be (8) a hidden coefficient that describes the relation of
%
$$\text{slo fulfillment} \sim \frac{\text{resource demand}}{\text{resource capacity}}$$
%
but I'm not sure yet to what extent we can learn this during the operation, or just visualize it as part of the evaluation.
% \ins{What is actually required to answer the first point? Do we want to go into BNL again, or are there some nice alternatives? Also from the exploration perspective we have a number of options that we should consider, however, I have the feeling that our platoon is still small compared to complex graphs that are usually tackled with heuristics, etc.}

While MKP provides an efficient way to model the problem, the agent must still provide the expected SLO fulfillment and resource demand so that the problem can be solved, either through DP or MILP. A solution here might be that we don't have to provide the values for all combinations, but either approximate them as well as possible or simply disregard them if the agent is not willing to explore further, e.g., if SLOs are sufficiently fulfilled with known choices. But whenever the leader sees the necessity, it can hold experiments through the following process: (1) find a device with idle resources, (2) deploy a service there, and (3) observe the resource demand and the SLO fulfillment. In case (4) the experiment shows implications on the regular device operations or the leader decides that enough data was collected, the experiment is terminated. 

% \rw{This time I would also not include dynamic adaptations of the service, e.g., change the streaming resolution to match the SLO fulfillment, but just include the parameters as part of the SLO. The agent might then find out through Q learning that choosing another configuration within its options actually improves the SLO fulfillment. However, this would change the value function of assigning a certain service to a host, which we will have to model somehow.}

Based on the gathered knowledge, the leader can infer that it would be advisable to offload computation from a source device to a target device, which unfolds the following process: (1) start executing the service at the target device parallel to the source device and (2) ensuring that the target device fulfills SLOs, i.e., according to the reported metrics. Only in case the SLO fulfillment is guaranteed at the target device, (3) the result of the target device is supplied to the original recipient, and (4) service execution is stopped at the origin device. 

% \ins{If I really want to include the graceful offloading, I must provide a bit more ideas here and also hint this in the problem description.}

% This is what I was talking about with Prof. Liang Wang, that I must first ensure that the second location is capable of running the service before I actually offload the computation. However, I would not dive too much into technical streaming implementations but rather focus on the concept that we start the execution in parallel and evaluate how it's running.

\subsection*{Evaluation}

To show the technical feasibility of our approach, we develop a prototype of the methodology and underline our contributions by conducting experiments. The prototype will be mainly implemented in Python and contain the actual services for video and point cloud processing, which are continuously evaluated according to SLOs; further, it contains the exploration mechanism and the graceful offloading of continuous streams.
%
The prototype will be executed and evaluated on the numerous Jetson devices that we have available, among them the three Orin NX from the cars and the one I have extra; in case we want more heterogeneity, we can also include the Orin AGX and a regular Nano, or put the devices in different operation modes. The selected devices will form the platoon, which will communicate with each other through the local network (or IBSS).

The scenarios we want to show within the experiments are (1) a platoon member is capable of running computations locally to a satisfying degree, (2) it is incapable of doing so either due to (2.1) violated QoE or (2.2) violated energy consumption, (3) the platoon member evaluates whether there exist other members that could spare sufficient resources, (4) the member finds a fitting location and the processing there (4.1) goes well as expected, or (4.2) encounters problems, which require further offloading.

The part of the solution that can best be compared with existing solutions is the decision-making for the offloading, which can include some heuristics or shortest-path methods as baselines; we might even compare it with brute-force testing for viable solutions. I don't think that its feasible to compare the SLO fulfillment with existing research because they did not evaluate this. \rw{Apart from that, we can compare the SLO fulfillment with other setups that would utilize cloud resources for offloading, which supposedly are not able to satisfy latency constraints to the same extent}. The first point underlines the viability of our exploration mechanism to satisfy SLOs, \rw{the latter underlines the general necessity to offload to the edge}.

~

I must show that the CPU/GPU load is not linear if we assign $n$ services to the vehicle.

Maybe I could also show that if I put the energy SLO very well and we have an optional Yolo service running on the other vehicles, these tend to kill this service if there are not enough resources expected. This might actually be a contribution because this hierarchy avoids offloading services in a "ping-pong" manner between members.

I might compare the fuzzy adaptation with the classical logic


\subsection*{Limitations}

In the context of this paper, we assume a limited number of services and device types, which makes it still feasible to evaluate them individually without the need to generalize from one service to another. In case the number of services grows high, it's possible to extrapolate between the performance of services within the same category (e.g., CV task) according to their metadata, as done in \cite{sedlak_markov_2024}.

Further, we assume that SLOs (or rather their thresholds) maintain constant during the service executions; otherwise, the underlying value functions for the SLO fulfillment would change accordingly. Although this could be modeled as part of the solution, we do not see the need for dynamic updates in SLO thresholds within the context of this paper and leave this for future work.
